Multi-Perspective, Simultaneous Embedding

We describe MPSE: a Multi-Perspective Simultaneous Embedding method for visualizing high-dimensional data, based on multiple pairwise distances between the data points. Specifically, MPSE computes positions for the points in 3D and provides different views into the data by means of 2D projections (planes) that preserve each of the given distance matrices. We consider two versions of the problem: fixed projections and variable projections. MPSE with fixed projections takes as input a set of pairwise distance matrices defined on the data points, along with the same number of projections and embeds the points in 3D so that the pairwise distances are preserved in the given projections. MPSE with variable projections takes as input a set of pairwise distance matrices and embeds the points in 3D while also computing the appropriate projections that preserve the pairwise distances. The proposed approach can be useful in multiple scenarios: from creating simultaneous embedding of multiple graphs on the same set of vertices, to reconstructing a 3D object from multiple 2D snapshots, to analyzing data from multiple points of view. We provide a functional prototype of MPSE that is based on an adaptive and stochastic generalization of multi-dimensional scaling to multiple distances and multiple variable projections. We provide an extensive quantitative evaluation with datasets of different sizes and using different number of projections, as well as several examples that illustrate the quality of the resulting solutions.

==> 3D multiview graph visualization_arxiv_v3/figure_graph.tex <==

     \begin{table}[h!]
     \begin{center}
     \begin{tabular}{ | p{3cm} |c |c |c| }
     \hline

collaboration
&
 \includegraphics[width=0.2\textwidth]{figures/cred.png} 
      &
  \includegraphics[width=0.2\textwidth]{figures/cgreen.png}
      &
  \includegraphics[width=0.2\textwidth]{figures/cblue.png}
       \\ \hline

collaboration 3DMV
&
        \includegraphics[width=0.2\textwidth]{figures/graphs/col_r.png}
      &
          \includegraphics[width=0.2\textwidth]{figures/graphs/col_g.png}
      &
                   \includegraphics[ width=0.2\textwidth]{figures/graphs/col_b.png}
        \\ \hline
\includegraphics[width=0.2\textwidth]{figures/game_of_thrones.png}
Game of Thrones
&
   \includegraphics[width=0.2\textwidth]{figures/gtred.png}
      &
   \includegraphics[width=0.2\textwidth]{figures/gtgreen.png}
      &
   \includegraphics[width=0.2\textwidth]{figures/gtblue.png}
 
       \\ \hline
 
 
 
GT 3DMV
&
    \includegraphics[width=0.2\textwidth]{figures/graphs/gt_r.png}
      &
  \includegraphics[width=0.2\textwidth]{figures/graphs/gt_g.png}
      &
  \includegraphics[width=0.2\textwidth]{figures/graphs/gt_b.png}


        \\ \hline
  
      \end{tabular}
      \caption{ Analysis}
      \label{tbl:pic}
      \end{center}
      \end{table}



==> 3D multiview graph visualization_arxiv_v3/picture1.tex <==

     \begin{table}[h!]
     \begin{center}
     \begin{tabular}{ | p{3cm} |c |c |c|c| }
     \hline

123-12p1
&
 \includegraphics[width=0.1\textwidth]{figures/results2/cost123_12p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/123_12p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/123_12p1_coordinates_tmpprojection2.png}

           &
               
        \\ \hline

123-23p1
&
 \includegraphics[width=0.1\textwidth]{figures/results2/cost123_23p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/123_23p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/123_23p1_coordinates_tmpprojection2.png}

           &
               
        \\ \hline

123-13p1
&
 \includegraphics[width=0.1\textwidth]{figures/results2/cost123_13p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/123_13p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/123_13p1_coordinates_tmpprojection2.png}

           &
               
        \\ \hline

123-123p1
&
 \includegraphics[width=0.1\textwidth]{figures/results2/cost123_123p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/123_123p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/123_123p1_coordinates_tmpprojection2.png}

           &
               \includegraphics[width=0.1\textwidth]{figures/results2/123_123p1_coordinates_tmpprojection3.png}
        \\ \hline

123-12p2
&
 \includegraphics[width=0.1\textwidth]{figures/results2/cost123_12p2_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/123_12p2_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/123_12p2_coordinates_tmpprojection2.png}

           &
               
        \\ \hline

123-23p2
&
 \includegraphics[width=0.1\textwidth]{figures/results2/cost123_23p2_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/123_23p2_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/123_23p2_coordinates_tmpprojection2.png}

           &
               
        \\ \hline

123-13p2
&
 \includegraphics[width=0.1\textwidth]{figures/results2/cost123_13p2_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/123_13p2_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/123_13p2_coordinates_tmpprojection2.png}

           &
               
        \\ \hline

123-123p2
&
 \includegraphics[width=0.1\textwidth]{figures/results2/cost123_123p2_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/123_123p2_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/123_123p2_coordinates_tmpprojection2.png}

           &
               \includegraphics[width=0.1\textwidth]{figures/results2/123_123p2_coordinates_tmpprojection3.png}
        \\ \hline




      \end{tabular}
      \caption{ Fixed Projections}
      \label{tbl:pic1}
      \end{center}
      \end{table}





     \begin{table}[h!]
     \begin{center}
     \begin{tabular}{ | p{3cm} |c |c |c|c| }
     \hline


cluster-12p1
&
 \includegraphics[width=0.1\textwidth]{figures/results2/costcluster_12p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/cluster_cluster_12p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/cluster_cluster_12p1_coordinates_tmpprojection2.png}

           &
               
        \\ \hline

cluster-123p1
&
 \includegraphics[width=0.1\textwidth]{figures/results2/costcluster_123p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/cluster_cluster_123p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/cluster_cluster_123p1_coordinates_tmpprojection2.png}

           &
               \includegraphics[width=0.1\textwidth]{figures/results2/cluster_cluster_123p1_coordinates_tmpprojection3.png}
        \\ \hline

cluster-123p2
&
 \includegraphics[width=0.1\textwidth]{figures/results2/costcluster_123p2_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/cluster_cluster_123p2_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/cluster_cluster_123p2_coordinates_tmpprojection2.png}

           &
               \includegraphics[width=0.1\textwidth]{figures/results2/cluster_cluster_123p2_coordinates_tmpprojection3.png}
        \\ \hline

sqcirtr-12p1
&
 \includegraphics[width=0.1\textwidth]{figures/results2/costsqcirtr_12p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/edges_sqcirtr_12p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/edges_sqcirtr_12p1_coordinates_tmpprojection2.png}

           &
               
        \\ \hline

sqcirtr-12p2
&
 \includegraphics[width=0.1\textwidth]{figures/results2/costsqcirtr_12p2_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/edges_sqcirtr_12p2_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/edges_sqcirtr_12p2_coordinates_tmpprojection2.png}

           &
               
        \\ \hline

sqcirtr-123p1
&
 \includegraphics[width=0.1\textwidth]{figures/results2/costsqcirtr_123p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/edges_sqcirtr_123p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/edges_sqcirtr_123p1_coordinates_tmpprojection2.png}

           &
               \includegraphics[width=0.1\textwidth]{figures/results2/edges_sqcirtr_123p1_coordinates_tmpprojection3.png}
        \\ \hline

sqcirtr-123p2
&
 \includegraphics[width=0.1\textwidth]{figures/results2/costsqcirtr_123p2_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/edges_sqcirtr_123p2_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/edges_sqcirtr_123p2_coordinates_tmpprojection2.png}

           &
               \includegraphics[width=0.1\textwidth]{figures/results2/edges_sqcirtr_123p2_coordinates_tmpprojection3.png}
        \\ \hline

123old-123p1
&
 \includegraphics[width=0.1\textwidth]{figures/results2/cost123old_123p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/123old_123p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/123old_123p1_coordinates_tmpprojection2.png}

           &
               \includegraphics[width=0.1\textwidth]{figures/results2/123old_123p1_coordinates_tmpprojection3.png}
        \\ \hline

grid-12p1
&
 \includegraphics[width=0.1\textwidth]{figures/results2/costgrid_12p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/edges_grid_12p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/edges_grid_12p1_coordinates_tmpprojection2.png}

           &
               
        \\ \hline

grid-12p2
&
 \includegraphics[width=0.1\textwidth]{figures/results2/costgrid_12p2_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/edges_grid_12p2_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/edges_grid_12p2_coordinates_tmpprojection2.png}

           &
               
        \\ \hline


      \end{tabular}
      \caption{ Fixed Projections}
      \label{tbl:pic}
      \end{center}
      \end{table}



==> 3D multiview graph visualization_arxiv_v3/picture3.tex <==

     \begin{table}[h!]
     \begin{center}
     \begin{tabular}{ | p{3cm} |c |c |c|c| }
     \hline

proj123-123p2
&
 \includegraphics[width=0.1\textwidth]{figures/results3/costproj123_123p2_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results3/proj123_123p2_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results3/proj123_123p2_coordinates_tmpprojection2.png}

           &
               \includegraphics[width=0.1\textwidth]{figures/results3/proj123_123p2_coordinates_tmpprojection3.png}
        \\ \hline

projcluster-123p1
&
 \includegraphics[width=0.1\textwidth]{figures/results3/costprojcluster_123p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results3/cluster_projcluster_123p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results3/cluster_projcluster_123p1_coordinates_tmpprojection2.png}

           &
               \includegraphics[width=0.1\textwidth]{figures/results3/cluster_projcluster_123p1_coordinates_tmpprojection3.png}
        \\ \hline

projconfname-123p1
&
 \includegraphics[width=0.1\textwidth]{figures/results3/costprojconfname_123p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results3/projconfname_123p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results3/projconfname_123p1_coordinates_tmpprojection2.png}

           &
               \includegraphics[width=0.1\textwidth]{figures/results3/projconfname_123p1_coordinates_tmpprojection3.png}
        \\ \hline

projsqcirtr-123p2
&
 \includegraphics[width=0.1\textwidth]{figures/results3/costprojsqcirtr_123p2_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results3/edges_projsqcirtr_123p2_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results3/edges_projsqcirtr_123p2_coordinates_tmpprojection2.png}

           &
               \includegraphics[width=0.1\textwidth]{figures/results3/edges_projsqcirtr_123p2_coordinates_tmpprojection3.png}
        \\ \hline

proj123old-123p1
&
 \includegraphics[width=0.1\textwidth]{figures/results3/costproj123old_123p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results3/proj123old_123p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results3/proj123old_123p1_coordinates_tmpprojection2.png}

           &
               \includegraphics[width=0.1\textwidth]{figures/results3/proj123old_123p1_coordinates_tmpprojection3.png}
        \\ \hline

projgrid-12p1
&
 \includegraphics[width=0.1\textwidth]{figures/results3/costprojgrid_12p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results3/edges_projgrid_12p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results3/edges_projgrid_12p1_coordinates_tmpprojection2.png}

           &
               \includegraphics[width=0.1\textwidth]{figures/results3/edges_projgrid_12p1_coordinates_tmpprojection3.png}
        \\ \hline

projcupmouse-12p1
&
 \includegraphics[width=0.1\textwidth]{figures/results3/costprojcupmouse_12p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results3/projcupmouse_12p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results3/projcupmouse_12p1_coordinates_tmpprojection2.png}

           &
%               \includegraphics[width=0.1\textwidth]{figures/results3/projcupmouse_12p1_coordinates_tmpprojection3.png}
        \\ \hline


      \end{tabular}
          \caption{ variable projection }
      \label{tbl:pic}
      \end{center}
      \end{table}



==> 3D multiview graph visualization_arxiv_v3/picutre0.tex <==

     \begin{table}[h!]
     \begin{center}
     \begin{tabular}{ | c |c |c |c| }
     \hline
         \includegraphics[width=0.2\textwidth]{figures/results/costcirc_tri_p2_coordinates_tmp.png}
      & 
     \includegraphics[width=0.2\textwidth]{figures/results/circ_tri_p2_coordinates_tmpprojection1.png}
      & 
              \includegraphics[width=0.2\textwidth]{figures/results/circ_tri_p2_coordinates_tmpprojection2.png}
              
           & 
               \includegraphics[width=0.2\textwidth]{figures/results/circ_tri_p2_coordinates_tmpprojection3.png}
        \\ \hline
        
       
              \includegraphics[width=0.2\textwidth]{figures/results/costsculp_123p1_coordinates_tmp.png}
      & 
     \includegraphics[width=0.2\textwidth]{figures/results/sculp_123p1_coordinates_tmpprojection1.png}
      & 
              \includegraphics[width=0.2\textwidth]{figures/results/sculp_123p1_coordinates_tmpprojection2.png}
              
           & 
               \includegraphics[width=0.2\textwidth]{figures/results/sculp_123p1_coordinates_tmpprojection3.png}
        \\ \hline
  
  
  
  
   
   
              \includegraphics[width=0.2\textwidth]{figures/results/costsculp_123p2_coordinates_tmp.png}
      & 
     \includegraphics[width=0.2\textwidth]{figures/results/sculp_123p2_coordinates_tmpprojection1.png}
      & 
              \includegraphics[width=0.2\textwidth]{figures/results/sculp_123p2_coordinates_tmpprojection2.png}
              
           & 
               \includegraphics[width=0.2\textwidth]{figures/results/sculp_123p2_coordinates_tmpprojection3.png}
        \\ \hline
  
  
  
  
  
   
   
              \includegraphics[width=0.2\textwidth]{figures/results/costsculp_12p2_coordinates_tmp.png}
      & 
     \includegraphics[width=0.2\textwidth]{figures/results/sculp_12p2_coordinates_tmpprojection1.png}
      & 
              \includegraphics[width=0.2\textwidth]{figures/results/sculp_12p2_coordinates_tmpprojection2.png}
              
           & 
               \includegraphics[width=0.2\textwidth]{figures/results/sculp_12p2_coordinates_tmpprojection3.png}
        \\ \hline
  
  
  
  
  
   
   
              \includegraphics[width=0.2\textwidth]{figures/results/costsculp_123p1_coordinates_tmp.png}
      & 
     \includegraphics[width=0.2\textwidth]{figures/results/sculp_23p1_coordinates_tmpprojection1.png}
      & 
              \includegraphics[width=0.2\textwidth]{figures/results/sculp_23p1_coordinates_tmpprojection2.png}
              
           & 
               \includegraphics[width=0.2\textwidth]{figures/results/sculp_23p1_coordinates_tmpprojection3.png}
        \\ \hline
  
  
  
  
  
  
   
   
              \includegraphics[width=0.2\textwidth]{figures/results/costsculp_12p1_coordinates_tmp.png}
      & 
     \includegraphics[width=0.2\textwidth]{figures/results/sculp_12p1_coordinates_tmpprojection1.png}
      & 
              \includegraphics[width=0.2\textwidth]{figures/results/sculp_12p1_coordinates_tmpprojection2.png}
              
           & 
               \includegraphics[width=0.2\textwidth]{figures/results/sculp_12p1_coordinates_tmpprojection3.png}
        \\ \hline
  
  
  
  
  
  
        
      \end{tabular}
      \caption{ Analysis}
      \label{tbl:pic}
      \end{center}
      \end{table}
      


==> figure_graph.tex <==

     \begin{table}[h!]
     \begin{center}
     \begin{tabular}{ | p{3cm} |c |c |c| }
     \hline

collaboration
&
 \includegraphics[width=0.2\textwidth]{figures/cred.png} 
      &
  \includegraphics[width=0.2\textwidth]{figures/cgreen.png}
      &
  \includegraphics[width=0.2\textwidth]{figures/cblue.png}
       \\ \hline

collaboration 3DMV
&
        \includegraphics[width=0.2\textwidth]{figures/graphs/col_r.png}
      &
          \includegraphics[width=0.2\textwidth]{figures/graphs/col_g.png}
      &
                   \includegraphics[ width=0.2\textwidth]{figures/graphs/col_b.png}
        \\ \hline
\includegraphics[width=0.2\textwidth]{figures/game_of_thrones.png}
Game of Thrones
&
   \includegraphics[width=0.2\textwidth]{figures/gtred.png}
      &
   \includegraphics[width=0.2\textwidth]{figures/gtgreen.png}
      &
   \includegraphics[width=0.2\textwidth]{figures/gtblue.png}
 
       \\ \hline
 
 
 
GT 3DMV
&
    \includegraphics[width=0.2\textwidth]{figures/graphs/gt_r.png}
      &
  \includegraphics[width=0.2\textwidth]{figures/graphs/gt_g.png}
      &
  \includegraphics[width=0.2\textwidth]{figures/graphs/gt_b.png}


        \\ \hline
  
      \end{tabular}
      \caption{ Analysis}
      \label{tbl:pic}
      \end{center}
      \end{table}



==> picture1.tex <==

     \begin{table}[h!]
     \begin{center}
     \begin{tabular}{ | p{3cm} |c |c |c|c| }
     \hline

123-12p1
&
 \includegraphics[width=0.1\textwidth]{figures/results2/cost123_12p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/123_12p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/123_12p1_coordinates_tmpprojection2.png}

           &
               
        \\ \hline

123-23p1
&
 \includegraphics[width=0.1\textwidth]{figures/results2/cost123_23p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/123_23p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/123_23p1_coordinates_tmpprojection2.png}

           &
               
        \\ \hline

123-13p1
&
 \includegraphics[width=0.1\textwidth]{figures/results2/cost123_13p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/123_13p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/123_13p1_coordinates_tmpprojection2.png}

           &
               
        \\ \hline

123-123p1
&
 \includegraphics[width=0.1\textwidth]{figures/results2/cost123_123p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/123_123p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/123_123p1_coordinates_tmpprojection2.png}

           &
               \includegraphics[width=0.1\textwidth]{figures/results2/123_123p1_coordinates_tmpprojection3.png}
        \\ \hline

123-12p2
&
 \includegraphics[width=0.1\textwidth]{figures/results2/cost123_12p2_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/123_12p2_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/123_12p2_coordinates_tmpprojection2.png}

           &
               
        \\ \hline

123-23p2
&
 \includegraphics[width=0.1\textwidth]{figures/results2/cost123_23p2_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/123_23p2_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/123_23p2_coordinates_tmpprojection2.png}

           &
               
        \\ \hline

123-13p2
&
 \includegraphics[width=0.1\textwidth]{figures/results2/cost123_13p2_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/123_13p2_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/123_13p2_coordinates_tmpprojection2.png}

           &
               
        \\ \hline

123-123p2
&
 \includegraphics[width=0.1\textwidth]{figures/results2/cost123_123p2_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/123_123p2_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/123_123p2_coordinates_tmpprojection2.png}

           &
               \includegraphics[width=0.1\textwidth]{figures/results2/123_123p2_coordinates_tmpprojection3.png}
        \\ \hline




      \end{tabular}
      \caption{ Fixed Projections}
      \label{tbl:pic1}
      \end{center}
      \end{table}





     \begin{table}[h!]
     \begin{center}
     \begin{tabular}{ | p{3cm} |c |c |c|c| }
     \hline


cluster-12p1
&
 \includegraphics[width=0.1\textwidth]{figures/results2/costcluster_12p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/cluster_cluster_12p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/cluster_cluster_12p1_coordinates_tmpprojection2.png}

           &
               
        \\ \hline

cluster-123p1
&
 \includegraphics[width=0.1\textwidth]{figures/results2/costcluster_123p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/cluster_cluster_123p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/cluster_cluster_123p1_coordinates_tmpprojection2.png}

           &
               \includegraphics[width=0.1\textwidth]{figures/results2/cluster_cluster_123p1_coordinates_tmpprojection3.png}
        \\ \hline

cluster-123p2
&
 \includegraphics[width=0.1\textwidth]{figures/results2/costcluster_123p2_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/cluster_cluster_123p2_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/cluster_cluster_123p2_coordinates_tmpprojection2.png}

           &
               \includegraphics[width=0.1\textwidth]{figures/results2/cluster_cluster_123p2_coordinates_tmpprojection3.png}
        \\ \hline

sqcirtr-12p1
&
 \includegraphics[width=0.1\textwidth]{figures/results2/costsqcirtr_12p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/edges_sqcirtr_12p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/edges_sqcirtr_12p1_coordinates_tmpprojection2.png}

           &
               
        \\ \hline

sqcirtr-12p2
&
 \includegraphics[width=0.1\textwidth]{figures/results2/costsqcirtr_12p2_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/edges_sqcirtr_12p2_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/edges_sqcirtr_12p2_coordinates_tmpprojection2.png}

           &
               
        \\ \hline

sqcirtr-123p1
&
 \includegraphics[width=0.1\textwidth]{figures/results2/costsqcirtr_123p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/edges_sqcirtr_123p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/edges_sqcirtr_123p1_coordinates_tmpprojection2.png}

           &
               \includegraphics[width=0.1\textwidth]{figures/results2/edges_sqcirtr_123p1_coordinates_tmpprojection3.png}
        \\ \hline

sqcirtr-123p2
&
 \includegraphics[width=0.1\textwidth]{figures/results2/costsqcirtr_123p2_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/edges_sqcirtr_123p2_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/edges_sqcirtr_123p2_coordinates_tmpprojection2.png}

           &
               \includegraphics[width=0.1\textwidth]{figures/results2/edges_sqcirtr_123p2_coordinates_tmpprojection3.png}
        \\ \hline

123old-123p1
&
 \includegraphics[width=0.1\textwidth]{figures/results2/cost123old_123p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/123old_123p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/123old_123p1_coordinates_tmpprojection2.png}

           &
               \includegraphics[width=0.1\textwidth]{figures/results2/123old_123p1_coordinates_tmpprojection3.png}
        \\ \hline

grid-12p1
&
 \includegraphics[width=0.1\textwidth]{figures/results2/costgrid_12p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/edges_grid_12p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/edges_grid_12p1_coordinates_tmpprojection2.png}

           &
               
        \\ \hline

grid-12p2
&
 \includegraphics[width=0.1\textwidth]{figures/results2/costgrid_12p2_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results2/edges_grid_12p2_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results2/edges_grid_12p2_coordinates_tmpprojection2.png}

           &
               
        \\ \hline


      \end{tabular}
      \caption{ Fixed Projections}
      \label{tbl:pic}
      \end{center}
      \end{table}



==> picture3.tex <==

     \begin{table}[h!]
     \begin{center}
     \begin{tabular}{ | p{3cm} |c |c |c|c| }
     \hline

proj123-123p2
&
 \includegraphics[width=0.1\textwidth]{figures/results3/costproj123_123p2_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results3/proj123_123p2_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results3/proj123_123p2_coordinates_tmpprojection2.png}

           &
               \includegraphics[width=0.1\textwidth]{figures/results3/proj123_123p2_coordinates_tmpprojection3.png}
        \\ \hline

projcluster-123p1
&
 \includegraphics[width=0.1\textwidth]{figures/results3/costprojcluster_123p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results3/cluster_projcluster_123p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results3/cluster_projcluster_123p1_coordinates_tmpprojection2.png}

           &
               \includegraphics[width=0.1\textwidth]{figures/results3/cluster_projcluster_123p1_coordinates_tmpprojection3.png}
        \\ \hline

projconfname-123p1
&
 \includegraphics[width=0.1\textwidth]{figures/results3/costprojconfname_123p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results3/projconfname_123p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results3/projconfname_123p1_coordinates_tmpprojection2.png}

           &
               \includegraphics[width=0.1\textwidth]{figures/results3/projconfname_123p1_coordinates_tmpprojection3.png}
        \\ \hline

projsqcirtr-123p2
&
 \includegraphics[width=0.1\textwidth]{figures/results3/costprojsqcirtr_123p2_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results3/edges_projsqcirtr_123p2_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results3/edges_projsqcirtr_123p2_coordinates_tmpprojection2.png}

           &
               \includegraphics[width=0.1\textwidth]{figures/results3/edges_projsqcirtr_123p2_coordinates_tmpprojection3.png}
        \\ \hline

proj123old-123p1
&
 \includegraphics[width=0.1\textwidth]{figures/results3/costproj123old_123p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results3/proj123old_123p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results3/proj123old_123p1_coordinates_tmpprojection2.png}

           &
               \includegraphics[width=0.1\textwidth]{figures/results3/proj123old_123p1_coordinates_tmpprojection3.png}
        \\ \hline

projgrid-12p1
&
 \includegraphics[width=0.1\textwidth]{figures/results3/costprojgrid_12p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results3/edges_projgrid_12p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results3/edges_projgrid_12p1_coordinates_tmpprojection2.png}

           &
               \includegraphics[width=0.1\textwidth]{figures/results3/edges_projgrid_12p1_coordinates_tmpprojection3.png}
        \\ \hline

projcupmouse-12p1
&
 \includegraphics[width=0.1\textwidth]{figures/results3/costprojcupmouse_12p1_coordinates_tmp.png}
      &
     \includegraphics[width=0.1\textwidth]{figures/results3/projcupmouse_12p1_coordinates_tmpprojection1.png}
      &
              \includegraphics[width=0.1\textwidth]{figures/results3/projcupmouse_12p1_coordinates_tmpprojection2.png}

           &
%               \includegraphics[width=0.1\textwidth]{figures/results3/projcupmouse_12p1_coordinates_tmpprojection3.png}
        \\ \hline


      \end{tabular}
          \caption{ variable projection }
      \label{tbl:pic}
      \end{center}
      \end{table}



==> picutre0.tex <==

     \begin{table}[h!]
     \begin{center}
     \begin{tabular}{ | c |c |c |c| }
     \hline
         \includegraphics[width=0.2\textwidth]{figures/results/costcirc_tri_p2_coordinates_tmp.png}
      & 
     \includegraphics[width=0.2\textwidth]{figures/results/circ_tri_p2_coordinates_tmpprojection1.png}
      & 
              \includegraphics[width=0.2\textwidth]{figures/results/circ_tri_p2_coordinates_tmpprojection2.png}
              
           & 
               \includegraphics[width=0.2\textwidth]{figures/results/circ_tri_p2_coordinates_tmpprojection3.png}
        \\ \hline
        
       
              \includegraphics[width=0.2\textwidth]{figures/results/costsculp_123p1_coordinates_tmp.png}
      & 
     \includegraphics[width=0.2\textwidth]{figures/results/sculp_123p1_coordinates_tmpprojection1.png}
      & 
              \includegraphics[width=0.2\textwidth]{figures/results/sculp_123p1_coordinates_tmpprojection2.png}
              
           & 
               \includegraphics[width=0.2\textwidth]{figures/results/sculp_123p1_coordinates_tmpprojection3.png}
        \\ \hline
  
  
  
  
   
   
              \includegraphics[width=0.2\textwidth]{figures/results/costsculp_123p2_coordinates_tmp.png}
      & 
     \includegraphics[width=0.2\textwidth]{figures/results/sculp_123p2_coordinates_tmpprojection1.png}
      & 
              \includegraphics[width=0.2\textwidth]{figures/results/sculp_123p2_coordinates_tmpprojection2.png}
              
           & 
               \includegraphics[width=0.2\textwidth]{figures/results/sculp_123p2_coordinates_tmpprojection3.png}
        \\ \hline
  
  
  
  
  
   
   
              \includegraphics[width=0.2\textwidth]{figures/results/costsculp_12p2_coordinates_tmp.png}
      & 
     \includegraphics[width=0.2\textwidth]{figures/results/sculp_12p2_coordinates_tmpprojection1.png}
      & 
              \includegraphics[width=0.2\textwidth]{figures/results/sculp_12p2_coordinates_tmpprojection2.png}
              
           & 
               \includegraphics[width=0.2\textwidth]{figures/results/sculp_12p2_coordinates_tmpprojection3.png}
        \\ \hline
  
  
  
  
  
   
   
              \includegraphics[width=0.2\textwidth]{figures/results/costsculp_123p1_coordinates_tmp.png}
      & 
     \includegraphics[width=0.2\textwidth]{figures/results/sculp_23p1_coordinates_tmpprojection1.png}
      & 
              \includegraphics[width=0.2\textwidth]{figures/results/sculp_23p1_coordinates_tmpprojection2.png}
              
           & 
               \includegraphics[width=0.2\textwidth]{figures/results/sculp_23p1_coordinates_tmpprojection3.png}
        \\ \hline
  
  
  
  
  
  
   
   
              \includegraphics[width=0.2\textwidth]{figures/results/costsculp_12p1_coordinates_tmp.png}
      & 
     \includegraphics[width=0.2\textwidth]{figures/results/sculp_12p1_coordinates_tmpprojection1.png}
      & 
              \includegraphics[width=0.2\textwidth]{figures/results/sculp_12p1_coordinates_tmpprojection2.png}
              
           & 
               \includegraphics[width=0.2\textwidth]{figures/results/sculp_12p1_coordinates_tmpprojection3.png}
        \\ \hline
  
  
  
  
  
  
        
      \end{tabular}
      \caption{ Analysis}
      \label{tbl:pic}
      \end{center}
      \end{table}
      

